Generating Human Interaction Motions in Scenes with Text Control

We present TeSMo, a method for text-controlled scene-aware motion generation based on denoising diffusion models. Previous text-to-motion methods focus on characters in isolation without considering scenes due to the limited availability of datasets that include motion, text descriptions, and interactive scenes. Our approach begins with pre-training a scene-agnostic text-to-motion diffusion model, emphasizing goal-reaching constraints on large-scale motion-capture datasets. We then enhance this model with a scene-aware component, fine-tuned using data augmented with detailed scene information, including ground plane and object shapes. To facilitate training, we embed annotated navigation and interaction motions within scenes. The proposed method produces realistic and diverse human-object interactions, such as navigation and sitting, in different scenes with various object shapes, orientations, initial body positions, and poses. Extensive experiments demonstrate that our approach surpasses prior techniques in terms of the plausibility of human-scene interactions, as well as the realism and variety of the generated motions. Code will be released upon publication of this work at https://research.nvidia.com/labs/toronto-ai/tesmo.

==> sec/04_dataset.tex <==
\section{Dataset.}
\input{figtex/03_dataset}

% \subsection{Dataset.}
\paragraph{Loco-3D-FRONT.}
To train the scene-aware branch of our navigation model, we require a dataset featuring motions navigating through various scenes. We curate the Loco-3D-FRONT dataset by integrating all "walking" motions from HumanML3D into diverse 3D environments from \cite{fu20213d}. Each motion is placed within a different scene with randomized initial translation and orientation, following the methodology outlined in \cite{yi2022mime}, as depicted in a) \fref{fig:dataset}. 
Additionally, we apply left-right flip data augmentation \cite{22cvpr_humanml3d} to both the motion and its interactive 3D scenes. Consequently, our dataset comprises approximately 11,000 walking motions, each accompanied by textual descriptions and 50 plausible 3D scenes.
% Existing captured motion dataset \cite{AMASS:ICCV:2019} does not have scenes. 
\paragraph{Interaction dataset.}
For training the scene-aware branch of the interaction model, we utilize the SAMP dataset \cite{21iccv_samp}, which captures motions and interactive objects simultaneously. Specifically, we focus on "sitting" and "stand-up" interactions, featuring 80 "sitting" motion sequences from the SAMP dataset interacting with chairs of varying heights.
% 
To diversify the interactive objects, we randomly select objects from 3D-FRONT \cite{fu20213d} to match the contact vertices on human poses in the original SAMP motion sequences. This matching is achieved using the contact loss and collision loss techniques outlined in MOVER \cite{yi2022mover}. It's worth noting that the original SAMP motion sequences are often lengthy, averaging around 100 seconds, and lack paired textual descriptions. For instance, a "sit" motion sequence typically involves walking toward an object, sitting down, and eventually standing up and moving away.
% 
To effectively learn human-object interaction skills, we extract sub-sequences containing human-object interactions, such as "walk/stand up to sit" and "stand up/walk from sitting." These sub-sequences consistently include sitting poses either at the beginning or end, accompanied by straightforward textual descriptions, e.g., "a person walks to an object and then sits." To enhance diversity, we incorporate style descriptions of sitting poses, such as "a person walks and sits down on a chair while crossing their arms."
% 
Applying left-right data augmentation to both motion and interactive objects results in approximately 200 different sub-sequences for each motion sequence, each paired with corresponding text descriptions and featuring various interactive objects, as illustrated in b) \fref{fig:dataset}.

\begin{comment}
We use SAMP \cite{21iccv_samp} dataset, which captures the motions and interactive objects simultaneously, to train the scene-aware branch of interaction model. Specifically, we only consider "sitting" and "stand-up" interactions. There are 80 ``sitting" motion sequences from SAMP dataset \cite{21iccv_samp}, interacting wiith four different chairs of different heights. 

To enrich the diversity of the interactive objects, we randomly select the objects from 3D-FRONT \cite{fu20213d} to match the contact vertices on the human poses in the original SAMP motion sequence, via the contact loss and collision loss in MOVER \cite{}.
% 
Note that, the original motion sequence in SAMP is quite long, the average length is 100s, and it does not have paired text.
For example, a ``sit'' motion sequence starts from a person far away from the object, first walk towards to the object, then sit down for a while, later stand up and go away. 
% 
To learn the useful human-object interaction ability, we need the motion clips that contains the human-object interaction, such as ``walk/stand up to sit" and ``stand up/walk from sitting". 
% 
Therefore, we extract the sub-sequences which always contain the sitting poses inside, either starting from the sitting pose or ending with sitting poses, and prepare the corresponding simple text description, such as ``a person walks to an object and then sit". To enrich the description, we also add sitting poses style description, such as ``a person walks and sit down on a chair while crosses his arms." 

Following the same left-right data augmentation for the motion and its interactive object, finally, each motion sequence results in around $200$ different sub-sequence with corresponding text description and different interactive objects, as shown in b) in \fref{fig:dataset}.
\end{comment}

==> tables/00_loco_motion.tex <==
% \begin{table}[ht]
% \begin{center}
% \begin{tabular}{|c|c|c|c|c|c|c|c|}
% \hline
% Method & Joint & FID & R-precision $\uparrow$ & Diversity $\rightarrow$ & Foot skating & Traj. err. & Loc. err. & Avg. err. $\downarrow$ \\
% \hline
% Real &  & 0.002 & 0.797 & 9.503 & 0.000 & 0.000 & 0.000 & 0.000 \\
% \hline
% PriorMDM & Pelvis & 0.698 & 0.602 & 9.197 & 0.1019 & 0.4022 & 0.3076 & 0.5959 \\
% \cline{2-9}
% & All & 0.475 & 0.583 & 9.156 & 0.0897 & 0.3457 & 0.2132 & 0.4417 \\
% \hline
% GMD & Pelvis & 0.576 & 0.665 & 9.206 & 0.1009 & 0.0931 & 0.0321 & 0.1439 \\
% \cline{2-9}
% & All & 0.218 & 0.687 & 9.422 & 0.0547 & 0.0387 & 0.0096 & 0.0338 \\
% \hline
% OminControl & Pelvis & 0.322 & 0.691 & 9.545 & 0.0571 & 0.0404 & 0.0085 & 0.0367 \\
% \cline{2-9}
% OminControl & Average & 0.310 & 0.693 & 9.502 & 0.0608 & 0.0617 & 0.0107 & 0.0404 \\

% \hline
% Ours & Pelvis & 0.322 & 0.691 & 9.545 & 0.0571 & 0.0404 & 0.0085 & 0.0367 \\

% \hline
% \end{tabular}
% \caption{Quantitative results on the HumanML3D test set. Ours (on pelvis) means the model is
% only trained on pelvis control. Joint (Average) reports the average performance over all joints. means closer to real data is better. }
% \end{center}
% \end{table}
% \resizebox{\columnwidth}{
\begin{table*}
\begin{center}
\caption{
% \todo{We probably should not evaluate this results, first, our trajectory generation is conditioned on the start position and end position which is too sparse compared with other methods, so the generated trajectory could be far away from the gt. second, it's for evaluating the generated motion that follows the input text, since we just take the other method as input, the evaluation in Omnicontrol is already clear to show the difference. I want to evaluate the feet skating to measure how realism our generated loco motion is.}
[Realism.] Controllable locomotion generation evaluation. 
% \todo{we can use a floor map as an empty space, and try our method.}
Quantitative results on the HumanML3D test set. 
Evaluation on the whole generated loco-motion.
Ours (on pelvis) means the model is trained only on pelvis control. Joint (Average) reports the average performance over all joints. ``$\rightarrow$'' indicates that a lower value is better, while ``$\uparrow$'' indicates that a higher value is better.}
\label{table:loco_cmp}

% \resizebox{\textwidth}{!}{%
\begin{tabular}{c|cccc|c}
\hline
Method & Joint & FID $\downarrow$ & R-precision $\uparrow$ & Diversity $\uparrow$ & Foot skating $\downarrow$ \\
% \hline
% \multicolumn{9}{c}{overall loco-motion} \\
Real {GT} &  & 0.0096 & 0.6717 & 7.5525 & 0.000 \\ \hline
% PriorMDM \cite{priormdm} &  & 78.515 & 0.4168 & 6.6328 & 0.0575 \\ \hline

% PriorMDM \cite{priormdm} &  & 7.8515 & 0.4168 & 6.6328 & 0.0575 \\ \hline

% % \hline

% MDM \cite{} & Pelvis & 0.698 & 0.602 & 9.197 & 0.1019 & 0.4022 & 0.3076 & 0.5959 & \\
% GMD\cite{} & Pelvis & 0.576 & 0.665 & 9.206 & 0.1009 & 0.0931 & 0.0321 & 0.1439 & \\
% PriorMDM\cite{} & Pelvis & 0.475 & 0.583 & 9.156 & 0.0897 & 0.3457 & 0.2132 & 0.4417 & \\
% OmniControl\cite{} (on pelvis) & Pelvis & 0.218 & 0.687 & 9.422 & 0.0547 & 0.0387 & 0.0096 & 0.0338 & \\
% OmniControl\cite{} (on all) & Pelvis & 0.322 & 0.691 & 9.545 & 0.0571 & 0.0404 & 0.0085 & 0.0367 & \\
% \hline
% \hline
% \\
% \multicolumn{9}{c}{overall loco-motion with our generated trajectory [test split]} \\
% GMD (start, end position) \cite{karunratanakul2023gmd} & Pelvis & 0.576 & 0.665 & 9.206 & 0.1009  \\

GMD \cite{karunratanakul2023gmd} & Pelvis & \textbf{13.16} & 0.1140 & 4.4875 & 0.181 \\
% GMD \cite{karunratanakul2023gmd}* & Pelvis & - & - & - & 0.3156 \\
OmniControl\cite{xie2023omnicontrol}*  & Pelvis & 22.93 & \textbf{0.4579}  & \textbf{7.128} & 0.0937 \\
\hline
% \\
% DIMOS\cite{}(start, end position, <0.2m) &  & 0.475 & 0.583 & 9.156 & 0.0897 & 0.3457 & 0.2132 & 0.4417 & \\
% PriorMDM \cite{} & Pelvis &  &  &  &  &  &  & 0.4417 & \\
% A* + PriorMDM  & Pelvis &  &  &  &  \\
\textbf{Ours} (OmniControl\cite{xie2023omnicontrol}) & Pelvis & \textbf{17.927} & \textbf{0.396} & 6.288 & \textbf{0.0308} \\
\textbf{Ours} (PriorMDM \cite{priormdm}) \cite{} & Pelvis & 20.465 & 0.3757 & 6.4152 & 0.0563 \\
% \textbf{Ours} (PriorMDM+root) & Pelvis & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \\
\hline
\end{tabular}
% }
\end{center}
\end{table*}
% }

==> tables/03_user_study_loco_as.tex <==
\begin{table}
  \begin{minipage}[t]{0.45\textwidth}
    \centering
        \caption{Ablation study examining the impact of various inference guidance on navigation generation performance, focusing on goal-reaching accuracy and human-scene interaction.}
        \resizebox{\textwidth}{!}{
        \label{table:ablation_study}
        \begin{tabular}{c|cc}
        \hline
        % Method  & \multicolumn{2}{c}{Locomotion} & \multicolumn{2}{c}{Interaction} \\
        % 
        Method & Pos.\ err.\ ($\downarrow$) & Col.\ R.\ ($\downarrow$) \\
        \hline
        Ours & 0.1568 & 0.0294\\
        w. goal reaching & \textbf{0.118} &  0.0342\\
        w. collision & 0.1550 & 0.0013\\
        w. collision \& goal reaching & 0.1241 & \textbf{0.0012}
        \end{tabular}
        }
    \label{table:ablation_loco_guidance}
  \end{minipage}
  \hfill
  \begin{minipage}[t]{0.45\textwidth}
    \centering
    \caption{Comparison of user study results assessing preferences for generated interactive motions. Higher scores indicate better preference for plausible human-object interaction.}
    \label{tab:locomotion}
    \resizebox{0.4\textwidth}{!}{
    \begin{tabular}{c|c}
    \toprule
    Method & User Study $\uparrow$  \\
    \midrule
    % MDM &  \\
    % PriorMDM & \\
    DIMOS & 29.1 \% \\
    \hline
    Ours & \textbf{71.9 \%} \\
    % \bottomrule
    \end{tabular}
    }
    % \caption{Caption for Table 2}
    \label{table:interaction_user_study}
  \end{minipage}

  % \begin{minipage}{0.45\textwidth}
    
  %   \begin{tabular}{cc}
  %   \toprule
  %   Method & User Study $\uparrow$  \\
  %   \midrule
  %   % MDM &  \\
  %   % PriorMDM & \\
  %   DIMOS & \\
  %   \hline
  %   Ours & \\
  %   \bottomrule
  %   \end{tabular}
  %   \bigskip\centering
  %   \end{minipage}
    
\end{table}


